Hardware Impairments Aware Transceiver Design for Full-Duplex Amplify-and-Forward MIMO Relaying

In this work we study the behavior of a full-duplex (FD) and amplify-and-forward (AF) relay with multiple antennas, where hardware impairments of the FD relay transceiver is taken into account. Due to the inter-dependency of the transmit relay power on each antenna and the residual self-interference in an FD-AF relay, we observe a distortion loop that degrades the system performance when the relay dynamic range is not high. In this regard, we analyze the relay function in presence of the hardware inaccuracies and an optimization problem is formulated to maximize the signal to distortion-plus-noise ratio (SDNR), under relay and source transmit power constraints. Due to the problem complexity, we propose a gradient-projection-based (GP) algorithm to obtain an optimal solution. Moreover, a nonalternating sub-optimal solution is proposed by assuming a rank-1 relay amplification matrix, and separating the design of the relay process into multiple stages (MuStR1). The proposed MuStR1 method is then enhanced by introducing an alternating update over the optimization variables, denoted as AltMuStR1 algorithm. It is observed that compared to GP, (Alt)MuStR1 algorithms significantly reduce the required computational complexity at the expense of a slight performance degradation. Finally, the proposed methods are evaluated under various system conditions, and compared with the methods available in the current literature. In particular, it is observed that as the hardware impairments increase, or for a system with a high transmit power, the impact of applying a distortion-aware design is significant.

==> AF_DF_Comparison.tex <==
 In this part, we study the performance of the defined system, assuming the relay decodes the interference-suppressed received signal, $ {r}_{{\rm supp},k}$, prior to amplification. As the result (2) can be formulated as 

\begin{align}
 {r}_{{\rm out},k} &= \underbrace{ a_k \cdot \rho \big ( {r}_{{\rm supp},k}  } \big) +  {e}_{{\rm out},k}, \\
 %{r}_{{\rm supp},k} &= { r}_{{\rm in},k} - {\tilde{h}}_{{\rm rr},k} \cdot {u}_{{\rm out},k},
\end{align}
where $\rho \big ( \cdot\big)$ represents the maximum likelihood decoder. The end-to-end rate of the relay channel can be hence calculated as 
\begin{align}
R_{\text{s-d},k} = \text{min} \big( R_{\text{s-r}} , R_{\text{r-d},k}  \big),
\end{align}
where  R_ is ...   .   Assuming gaussian dist. and following the previous studies in ... minimum gauranteed end to end rate for a given amplification coefficient a_k  can be formulated as 

log(1+omega_effective )

where omega_sr , omega_rd represent the  


Lemma 3: for the optimal choice of the amplification coefficietns, and also for an arbitrary, but equal choice of the amplification coefficient for the DF and AF cases, an increase in beta, gamma, or zetta, induces more error power in the AF scenario, compared t the FD case.


This provides us with an important indication, as the As the result 

==> _main_DF.tex <==
In the previous sections we studied the behavior of an AF-FD relay under residual self-interference, from the aspects of performance analysis and design methodologies. While an AF relaying is known to provide a simple strategy, it particularly suffers from the aforementioned distortion loop especially when the residual interference power is not ignorable, see~Subsection~\ref{discussion:distortionLoop}. In this part, we provide a similar study for a setup where the relay operates with DF protocol, in order to act as a comparison benchmark. In a DF relay, the discussed distortion loop is significantly alleviated as the decoding process eliminates the inter-dependency of the received residual interference intensity to the relay transmit signal power, see \cite[Section~V]{TRCM:15} for a similar discussion regarding single antenna relays. Note that optimization strategies for FD relays with DF process have been discussed in the literature, see~\cite{XaZXMaXu:15, DMBSR:12,ALRWW:14,RVRWW:15}, for different relaying setups and assumptions. In order to adopt the available literature to our setup, we follow a modified version of the approach given in \cite{ALRWW:14, RVRWW:15}, where an SDNR maximization problem is studied at a MIMO DF relay. Note that the proposed design in \cite{ALRWW:14,RVRWW:15} considers a maximization of the SDNR at the relay input/output, taking advantage of spatial and temporal filters. In our system, we focus on the resulting performance from the source to the destination, after the application of the receive filter $\ma{z}$, and hence including $P_{\text{s}}$ and $\ma{z}$ as optimization variables. Afterwards, similar to \cite{RVRWW:15}, we propose a joint optimization where in each step one of the variables is updated to the optimality. A detailed model update and design strategy is given in the following. 

\subsection{DF Relaying} We define $\ma{v}_{\text{in}} \in \compl^{M_{\text{r}}}$ as linear filter at the relay input, $\hat{s}_{\text{r}} \in \compl$, $\mathbb{E}\{|\hat{s}_{\text{r}}|^{2}\}=1$ as the decoded symbol, and $\ma{v}_{\text{out}} \in \compl^{M_{\text{t}}}$ as the beamforming vector to transmit the decoded data symbol, see Fig.~\ref{fig:DF_relay}. The end-to-end rate maximization can be equivalently formulated as 
\begin{subequations} \label{eq_DF_Op_array} 
\begin{align}  
\underset{\ma{v}_{\text{in}}, \ma{z}, \ma{Q}\in \mathcal{H}, P_{\text{s}} }{\text{max}} \;\; & \text{min} \left( \zeta_{\text{sr}}, \zeta_{\text{rd}} \right), \;\; \label{eq_DF_Op_a} \\ 
\text{s.t.} \;\;\;\;\;\; &\text{tr}\left( \ma{Q} \right) \leq \tilde{P}_{\text{r,max}}, \;P_{\rm {s}} \leq P_{\text{s,max}},\; \text{rank}(\ma{Q}) = 1,\label{eq_DF_Op_b}
\end{align}
\end{subequations}
where the rank-one constraint is imposed to ensure the structure $\ma{Q}:=\mathbb{E} \{ \ma{u}_{{\rm out}} \ma{u}_{{\rm out}}^{{H}} \} = \ma{v}_{\rm out} \ma{v}_{\rm out}^{H}$. The values $\zeta_{\text{sr}}$ and $\zeta_{\text{rd}}$, respectively represent the resulting SDNR in source-to-relay and relay-to destination links which can be calculated as 
\begin{align} 
\zeta_{\text{sr}} & \approx \frac{ P_{\text{s}}\ma{v}_{\text{in}}^H  \ma{h}_{{\rm sr}} \ma{ h}_{{\rm sr}}^H \ma{v}_{\text{in}} }{ \hspace{-0.5mm} \ma{v}_{\text{in}}^H  \Big( \sigma_{\text{nr}}^2 \ma{I}_{M_{\text{r}}} \hspace{-0.9mm} + \hspace{-0.9mm} \kappa \ma{H}_{\text{rr}} \text{diag} (\ma{Q}) \ma{H}_{\text{rr}}^H  \hspace{-0.9mm} +  \hspace{-0.9mm} \beta \text{diag} \left(\ma{H}_{\text{rr}} \ma{Q} \ma{H}_{\text{rr}}^H  \right) \hspace{-0.9mm} \Big) \ma{v}_{\text{in}}} ,\label{eq_DF_SINRsr}  \\
\zeta_{\text{rd}} & = \frac{ \ma{z}^H  \ma{H}_{\text{rd}} \ma{Q}  \ma{H}_{\text{rd}}^H \ma{z} }{\ma{z}^H  \Big(\sigma_{\text{nd}}^2 \ma{I}_{M_{\text{d}}}  + \kappa \ma{H}_{\text{rd}} \text{diag} (\ma{Q}) \ma{H}_{\text{rd}}^H + P_{\text{s}} \ma{h}_{\text{sd}}\ma{h}_{\text{sd}}^H\Big)  \ma{z}}. \label{eq_DF_SINRrd} 
\end{align}  
where the approximation in (\ref{eq_DF_SINRsr}) follows considering the fact that the self-interference signal constitutes the dominant part of the power in $\ma{u}_{{\rm in}}$, and can be regarded as the only cause of distortion signals at the relay, see also (\ref{eq_loop_U_in}). 
%It is easy to observe that at the source power constraint is necessarily tight at the optimality, as both $\zeta_{\text{sr}}$ and $\zeta_{\text{rd}}$ are monotonically increasing with respect to $P_{\text{s}}$. 
Note that (\ref{eq_DF_Op_array}) is not a convex optimization problem, and also can not be solved in a closed form. Nevertheless, recognizing the generalized Rayleigh quotient structure in (\ref{eq_DF_SINRsr}), (\ref{eq_DF_SINRrd}) we obtain 
\begin{align} 
\ma{z}^{\star} & =   \Big( \sigma_{\text{nd}}^2 \ma{I}_{M_{\text{d}}}  + \kappa \ma{H}_{\text{rd}} \text{diag} (\ma{Q}) \ma{H}_{\text{rd}}^H  +  P_{\text{s}} \ma{h}_{\text{sd}}\ma{h}_{\text{sd}}^H\Big)^{-1} \ma{H}_{\text{rd}} \ma{v}_{\text{out}} , \label{eq_DF_z_star}\\
\ma{v}_{\text{in}}^{\star} & =  \Big( \sigma_{\text{nr}}^2 \ma{I}_{M_{\text{r}}}  + \kappa \ma{H}_{\text{rr}} \text{diag} (\ma{Q}) \ma{H}_{\text{rr}}^H +  \beta \text{diag} \left(\ma{H}_{\text{rr}} \ma{Q} \ma{H}_{\text{rr}}^H  \right) \Big)^{-1} \nonumber \\ & \;\;\;\;\;\;\;\;\;\; \times \ma{h}_{\text{sr}}\sqrt{P_{\text{s}}}   , \label{eq_DF_v_in_star}
\end{align}  
where $\ma{z}^{\star}$, $\ma{v}_{\text{in}}^{\star}$ represent the optimum $\ma{z}$, $\ma{v}_{\text{in}}$ for a fixed $\ma{Q}$ and $P_{\text{s}}$. In order to obtain the optimal $\ma{Q}, P_{\text{s}}$, the problem in (\ref{eq_DF_Op_array}) can be re-formulated as 
\begin{subequations} \label{eq_DF_opt_Ps_Q}
\begin{align} 
\underset{ P_{\text{s}}, \zeta \in \real^+, \ma{Q}\in \mathcal{H} }{\text{max}} \;\; & \zeta \label{eq_DF_Op2_A}  \\
\text{s.t.} \;\;\;\;\;\;\; & \zeta \leq \zeta_{\text{sr}} , \; \zeta \leq \zeta_{\text{rd}} , \label{eq_DF_Op2_B}  \\
&\ma{Q}\in \mathcal{H}, \; \text{tr}\left( \ma{Q} \right) \leq \tilde{P}_{\rm{r,max}}, \; \text{rank}(\ma{Q}) = 1, \label{eq_DF_Op2_C} 
\end{align}
\end{subequations} 
where the values of $\ma{v}_{\text{in}}$ and $\ma{z}$ are fixed. By temporarily relaxing the rank constraint, the above problem can be written as a convex feasibility check over $\ma{Q} , P_{\text{s}}$, for each value of $\zeta$ as 
\begin{subequations} \label{eq_DF_Op3_array}
\begin{align} 
{\text{find}} \;\; & \ma{Q}, P_{\text{s}} \label{eq_DF_Op3_a}  \\
\text{s.t.} \;\; & \text{tr}\left( \ma{Q} \right) \leq \tilde{P}_{\text{r,max}},\;\;  P_{\text{s}} \geq 0,\;  \ma{Q}\in \mathcal{H}, \label{eq_DF_Op3_d} \\
%&  \label{eq_DF_Op3_c}  \\
&   \text{tr}\left( {\ma{\Psi}}_{\text{sr}} +  {\ma{\Phi}}_{\text{sr}} \ma{Q}  \right) \geq 0, \; \text{tr}\left( {\ma{\Psi}}_{\text{rd}} +  {\ma{\Phi}}_{\text{rd}} \ma{Q}  \right) \geq 0, \label{eq_DF_Op3_b}   
\end{align}
\end{subequations} 
where
\begin{align} \label{eq_DF_PsiPhi} 
{\ma{\Psi}}_{\text{rd}} &:=  - \zeta  \ma{z}\ma{z}^H \left( \sigma_{\text{nd}}^2 \ma{I}_{M_{\text{d}}} + {P}_{\text{s}} \ma{h}_{{\text{sd}}} \ma{h}_{{\text{sd}}}^H \right) \\
{\ma{\Psi}}_{\text{sr}} &:= \ma{v}_{\text{in}}\ma{v}_{\text{in}}^H \left( {P}_{\text{s}} \ma{h}_{{\text{sr}}} \ma{h}_{{\text{sr}}}^H  - \zeta \sigma_{\text{nr}}^2 \ma{I}_{M_{\text{r}}}  \right), \\
{\ma{\Phi}}_{\text{rd}} &:=  \ma{H}_{{\text{rd}}}^H \ma{z} \ma{z}^H \ma{H}_{{\text{rd}}} - \zeta  \kappa \text{diag} \left( \ma{H}_{{\text{rd}}}^H \ma{z}\ma{z}^H \ma{H}_{{\text{rd}}} \right)  , \\
{\ma{\Phi}}_{\text{sr}} &:= -\zeta  \left( \kappa \text{diag} \left( \ma{H}_{{\text{rr}}}^H \ma{v}_{\text{in}}\ma{v}_{\text{in}}^H \ma{H}_{{\text{rr}}} \right) + \beta \ma{H}_{{\text{rr}}}^H \text{diag} \left( \ma{v}_{\text{in}}\ma{v}_{\text{in}}^H \right) \ma{H}_{{\text{rr}}} \right).
\end{align}
Note that the iterations of the defined feasibility check will be continued, following a bi-section search procedure until an optimum $\zeta$ is obtained with sufficient accuracy. Fortunately, for the special structure of (\ref{eq_DF_Op3_array}) as a complex-valued semi-definite program with three linear constraints, we can always achieve an optimal rank-$1$ $\ma{Q}\in \mathcal{H}$, following \cite[Theorem~3.2]{PalomarSDPRank}. The optimal $\ma{v}_{\text{in}}$ is hence obtained as 
\begin{align} \label{eq_DF_v_out} 
\ma{v}_{\text{out}}^\star = {\ma{Q}^{\star}}^{\frac{1}{2}},   
\end{align}
where $\ma{Q}^{\star}$ represents the obtained $\ma{Q}$ for the highest feasible $\zeta$. It is worth mentioning that the feasible values of $\zeta$ is necessarily located in the region $[0, \zeta_{\text{max}}]$ where 
\begin{align} \label{eq_DF_zeta_max} 
\zeta_{\text{max}} := \text{min}  \left\{ \frac{{P}_{\text{s,max}} \|\ma{h}_{{\rm sr}}\|_2^2}{\sigma_{\text{nr}}^2} ,  \frac{ {P}_{\text{r,max}} \lambda_{\text{max}} \left\{ \ma{H}_{{\text{rd}}}\ma{H}_{{\text{rd}}}^H\right\} }{\sigma_{\text{nd}}^2} \right\}
\end{align}
corresponds to the minimum of the individual link qualities, assuming $\beta=\kappa=0$, and will be used as the initial bounds for the aforementioned bi-section search. The iterations of the defined optimization steps is continued until a stable point is obtained, or a pre-defined number of iterations is expired. Note that the solutions in (\ref{eq_DF_z_star})-(\ref{eq_DF_v_out}), result in a necessary improvement of $\zeta$, since in each step the defined sub-problem is solved to optimality. Moreover, since the performance of the studied relay system is bounded from above, see~(\ref{eq_DF_zeta_max}), the defined iterative update results in a necessary convergence. Algorithm~\ref{algorithm:DF} provides a detailed procedure. 


\begin{algorithm}[H]
 \small{	\begin{algorithmic}[1]
  %\SetAlgoLined
\State{$P_{\rm s} \leftarrow  P_{\text{s,max}} \times 10^{-2}  $}
\State{$\text{counter}_{1} \leftarrow 0$}
\Repeat    $\;\; \text{(main optimization steps)}$
\State{$\text{counter}_{1} \leftarrow \text{counter}_{1} + 1$}
\State{$\ma{v}_{\text{in}} \leftarrow \ma{v}_{\text{in}}^{\star}, \;\; \text{see~(\ref{eq_DF_v_in_star})}$}
\State{$\ma{z} \leftarrow \ma{z}^{\star}, \;\; \text{see~(\ref{eq_DF_z_star})}$}
\State{$\text{counter}_{2} \leftarrow 0$}
\State{$\zeta_{\text{min}} \leftarrow 0$}
\State{$\zeta_{\text{max}} \leftarrow \text{see~(\ref{eq_DF_zeta_max})} $}
\Repeat   $\;\; \text{(bi-section search steps)}$
\State{$\zeta \leftarrow (\zeta_{\text{min}} + \zeta_{\text{max}})/2$}
\If{\text{(\ref{eq_DF_Op3_a})-(\ref{eq_DF_Op3_d}) is feasible}}
\State{$\zeta_{\text{min}} \leftarrow \zeta$}
\Else 
\State{$\zeta_{\text{max}} \leftarrow \zeta$}
\EndIf
\Until {$\text{counter}_2 \leq C_2 $ }
\State{$\zeta^{\text{counter}_1}  \leftarrow (\zeta_{\text{min}} + \zeta_{\text{max}})/2$}
\State{$P_{\text{s}} \leftarrow P_{\text{s}}^{\star}, \;\; \text{see~(\ref{eq_DF_opt_Ps_Q})}$}
\State{$\ma{v}_{\text{out}} \leftarrow \ma{v}_{\text{out}}^{\star}, \;\; \text{see~(\ref{eq_DF_v_out})}$}
\Until {$\text{counter}_1 \leq C_1 \;\; \text{or}\;\; \zeta^{\text{counter}_1} - \zeta^{\text{counter}_1-1} \leq {c}_1$ }
\State{\Return{$\left(P_{\text{s}},\ma{z},\ma{v}_{\text{in}},\ma{v}_{\text{our}},\right)$}}%%%
  \end{algorithmic}  
 \caption{\small{An iterative rate maximization algorithm for decode-and-forward relaying. $C_1,C_2 \in \mathbb{N}$ respectively represent the number of the main optimization steps and the bi-section process, and ${c}_1 \in \real^+$ determines the stability condition.} }  \label{algorithm:DF} } 
\end{algorithm}  





\begin{figure}[t]  
{\includegraphics[angle = 0, width = 0.99\columnwidth]{DF_model.pdf}} 
%\LoadClass[onecolumn]{article}
%\addtolength{\linewidth}{3.6in}
\caption{\footnotesize{A schematic of a decode-and-forward relaying process. $\rho\{\cdot\}$ and $\hat{s}_{\text{r}}$ represent the decoding process, and the estimate of the transmitted symbol, $s$, at the relay. The receive and transmit spatial filters are represented as $\ma{v}_{\text{in}}$ and $\ma{v}_{\text{out}}$, respectively. The bold arrows represent the vector signals while the dashed arrows represent the scalars. }} 
\label{fig:DF_relay}
\end{figure}

==> macros.tex <==
\usepackage{bm}
%=== symbols =====================================================
%\newcommand{\ma}[1]{\bm{ #1 }}         % matrix/vector
\newcommand{\ma}[1]{\mathbf{ #1 }}         % matrix/vector

\newcommand{\ten}[1]{\ma{\mathcal #1}} % tensor
\newcommand{\set}[1]{{\mathcal #1}}    % set

\newcommand{\compl}{\mathbb{C}}        % complex-valued numbers
\newcommand{\real}{\mathbb{R}}         % real-valued numbers

\newcommand{\eqdef}{\stackrel{.}{=}} % definition


%=== functional operators ======================================
\newcommand{\realof}[1]{{\rm Re}\left\{ #1 \right\}}           % real part
\newcommand{\imagof}[1]{{\rm Im}\left\{ #1 \right\}}           % imaginary part
\newcommand{\vecof}[1]{{\rm vec}\left\{ #1 \right\}}           % vec operator
\newcommand{\unvecof}[2]{\mathop{\rm unvec}_{#2}\left\{ #1 \right\}}% unvec operator
\newcommand{\diagof}[1]{{\rm diag}\left\{ #1 \right\}}         % diag operator
\newcommand{\traceof}[1]{{\rm tr}\left\{ #1 \right\}}          % trace operator
\newcommand{\twonorm}[1]{\left\|#1\right\|_2}                  % two-norm
\newcommand{\fronorm}[1]{\left\|#1\right\|_{\rm F}}            % Frobenius norm
\newcommand{\honorm}[1]{\left\|#1\right\|_{\rm H}}             % higher-order norm
\newcommand{\maxof}[1]{{\rm max} \left\{ #1 \right\}}          % max
\newcommand{\minof}[1]{{\rm min} \left\{ #1 \right\}}          % min
\newcommand{\expvof}[1]{\mathbb{E}\left\{ #1 \right\}}         % expected value
\newcommand{\expof}[1]{{\rm e}^{#1}}                           % e^{}


%=== other operators ===========================================
\newcommand{\argmax}{\mathop{{\arg \max}}}         % argmax

%=== binary operators ===========================================
\newcommand{\krp}{\diamond}  % Khatri-Rao product: A \krp B
\newcommand{\kron}{\otimes}  % Kronecker product: A \kron B



%=== superscripts ================================================
\newcommand{\degrees}{\circ}   % e.g., 90^\degrees
\newcommand{\trans}{{\rm T}}   % transpose: ^\trans
\newcommand{\herm}{{\rm H}}    % hermitian: ^\herm
\newcommand{\mtrans}{-{\rm T}} % inv.transpose: ^\mtrans
\newcommand{\mherm}{-{\rm H}}  % inv.hermitian: ^\mherm
\newcommand{\pinv}{+}          % pseudo-inverse: ^\pinv
\newcommand{\conj}{*}          % complex conjugate: ^\conj



%=== Tensor stuff ================================================
\newcommand{\tconcat}{\mbox{\Huge \textvisiblespace \hspace{-0.2ex}} \;}
\newcommand{\unf}[2]{\left[ \ten{#1} \right]_{(#2)}}
\newcommand{\unfnot}[2]{\left[ #1 \right]_{(#2)}}


%=== short-hand for colors =======================================
\usepackage{color}
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}

%=== short hand for TWR quantities ===============================
\newcommand{\UT}[1]{\textsf{UT$_#1$}}
\newcommand{\UTM}[2]{\textsf{UT$_#1^{(#2)}$}}
\newcommand{\RS}{{\textsf{RS}}}
\newcommand{\RSf}{\textsf{R}}
\newcommand{\MR}{M_{\rm R}}
\newcommand{\NR}{N_{\rm R}}
\newcommand{\NP}{N_{\rm P}}
\newcommand{\NPi}[1]{N_{\rm P,#1}}
\newcommand{\PT}[1]{P_{{\rm T},#1}}
\newcommand{\PN}[1]{P_{{\rm N},#1}}
\newcommand{\PTR}{P_{{\rm T,R}}}
\newcommand{\PNR}{P_{{\rm N,R}}}
\newcommand{\PTx}{P_{{\rm T}}}
\newcommand{\PNx}{P_{{\rm N}}}

\newcommand{\eff}{{\rm (e)}}
\newcommand{\effT}{{\rm (e)^\trans}}
\newcommand{\effS}{{\rm (e)^2}}
\newcommand{\eq}{{\rm (eq)}}

\newcommand{\target}{{\rm (T)}}

\newcommand{\forw}{{\rm (f)}}
\newcommand{\forwT}{{\rm (f)^\trans}}
\newcommand{\forwH}{{\rm (f)^\herm}}
\newcommand{\backw}{{\rm (b)}}
\newcommand{\backwT}{{\rm (b)^\trans}}
\newcommand{\backwH}{{\rm (b)^\herm}}

\newcommand{\forwn}{{\rm (f,0)}}
\newcommand{\backwn}{{\rm (b,0)}}


%=== pseudo code =================================================
%\newcommand{\algorithmicinitiate}{\textbf{Initiate:}}

%=== other stuff =================================================
\newcommand{\note}[1]{\red{\bfseries #1}}
\newcommand{\TODO}[1]{\par\red{\bfseries ***TODO: #1***}\\}


==> main_Opt_AF.tex <==
In this section we obtain an optimal relay selection strategy together with the optimal relay amplification coefficients, following the max-min approach. This leads to the maximum end to end communication rate which is preserved for all multicast destination nodes, and for all feasible self-interference channel estimation errors defined by the sets $\mathcal{H}_k$ . Due to the single stream setup we equivalently define our problem as Signal-to-Error-plus-Noise-Ratio (SENR) maximization at the destination nodes. This can be hence formulated as 
\begin{align}
 \underset{k \in \mathbb{S}_K, \; a_k \in {\mathcal A}_k }{ \rm max }\;\; \big \{ \underset{n \in \mathbb{S}_N,\;  \delta_k \in \mathcal{H}_k }{ \rm min } \;\;  {\rm SENR}_k^{(n)} \big \},
\end{align}
% or equivalently as
% \begin{align}
% \underset{k \in \mathbb{S}_K, \; a_k \in {\mathcal A}_k }{ \rm max }\;\; & t \nonumber \\
% {\rm s.t.} \;\;\;\;\;\;\;\; & \left\{ \underset{n \in \mathbb{S}_N } { \rm min } \;\;   {\rm SENR}_k^{(n)} \right \} \geq t,
% \end{align}
where ${\mathcal A}_k$ includes all values of $a_k$ which satisfy the $R_k$ transmit power constraint (8), and ${\rm SENR}_k^{(n)}$ is the resulting SENR at $D_n$ if $R_k$ is selected as the active relay node. In order to solve the above problem, in the first step, we derive an explicit formulation for the relay's transmit power which plays an important role in the formulation of SENR values. By incorporating (1), (4)-(7) into (2) and (3) we have \footnotemark[1]    \footnotetext[1]{The relay output signals, i.e., ${u}_{{\rm out},k}$ and ${r}_{{\rm out},k}$, are generated from the received signals in the previous symbol duration. The subsequent communicated symbols are assumed zero-mean and independent. The time (symbol) index is eliminated to simplify the notations. }
\begin{align}
\mathcal{E} & \{ {u}_{{\rm out},k}  {u}_{{\rm out},k}^{*} \}  
 = \left|a_k \right|^2  \Big(   P_s \left|  { h}_{{\rm sr},k} \right|^2 + M_k +  \mathcal{E} \{ {e}_{{\rm in},k} {e}_{{\rm in},k}^{*} \} \nonumber \\ &+ \mathcal{E} \{ {e}_{{\rm out},k} {e}_{{\rm out},k}^{*} \} \cdot \left|{ h}_{{\rm rr},k} \right|^2 + \mathcal{E} \{ {r}_{{\rm out},k} {r}_{{\rm out},k}^{*} \} \cdot \left|{ \delta}_{k} \right|^2  \Big) \nonumber \\
 & = \left|a_k \right|^2  \bigg( P_s \left|  { h}_{{\rm sr},k} \right|^2 + M_k +  \mathcal{E} \{ {u}_{{\rm in},k} {u}_{{\rm in},k}^{*} \}  \beta_k \nonumber \\  &+ \mathcal{E} \{ {u}_{{\rm out},k} {u}_{{\rm out},k}^{*} \} \cdot \left( \left|{ h}_{{\rm rr},k} \right|^2 \gamma_k + (1 + \gamma_k) |\delta_k|^2  \right)  \bigg), 
 \label{eq:u_out_power}
\end{align}
where $P_s:= \mathcal{E} \{ s s^{*} \}$ is the transmit power from the source. The undistorted received power at the relay can be calculated from (1)-(3) as 
\begin{align}
 \mathcal{E} \{ {u}_{{\rm in},k} {u}_{{\rm in},k}^{*} \} & =  P_s \left|  { h}_{{\rm sr},k} \right|^2 + M_k + \left|{ h}_{{\rm rr},k} \right|^2  \mathcal{E} \{ {r}_{{\rm out},k} {r}_{{\rm out},k}^{*} \}.
 \label{eq:approximation_power}
\end{align}
It is worth mentioning that due to the proximity of the Rx and Tx antennas on the FD device, the loopback self-interference signal is much stronger than the desired signal which is coming from a distant location, e.g., up to 100 dB according to [6], and hence constitutes the principle part in (12). By incorporating (12) into (11) and recalling (6) and (2) we have 
\begin{align}
 \mathcal{E} \{ {r}_{{\rm out},k} &  {r}_{{\rm out},k}^{*} \} \nonumber  \\
 & = \left( \gamma_k +1 \right) \cdot \mathcal{E} \{ {u}_{{\rm out},k}  {u}_{{\rm out},k}^{*} \}\nonumber \\
& = \frac{ \left( \eta_k +1 \right)  \left|a_k \right|^2  \left (P_s \left|  { h}_{{\rm sr},k} \right|^2 + M_k \right )   } {1 - \left|a_k \right|^2 \Big( \left|  { h}_{{\rm rr},k} \right|^2  \eta_k + (\gamma_k +1 ) \left|{ \delta}_{k} \right|^2  \Big) },
 \label{eq:tx_power}
\end{align}
where $\eta_k := \gamma_k + \beta_k +  \gamma_k\beta_k$. Note that the above derivations (11)-(13) hold given that all components of the desired signal ($s$), noise ($m_k$) and the distortion components (${e}_{{\rm in},k},{e}_{{\rm out},k}$) are zero mean and mutually independent. In order to obtain an explicit formulation for ${\rm SENR}_k^{(n)}$, we distinguish the desired as well as the error plus noise parts of the signal power at the destination. By exploiting the independence among noise, error and desired signal components we have
\begin{align}
P_{{\rm desired},k}^{(n)} &= P_s  \cdot \left|a_k \right|^2 \left|  { h}_{{\rm sr},k}  { h}_{{\rm rd},k}^{(n)} \right|^2    \label{eq:desired_power} \\
P_{{\rm destructive},k}^{(n)} &=  \left|  { h}_{{\rm rd},k}^{(n)}  \right|^2 \Big ( \mathcal{E} \{ {r}_{{\rm out},k}  {r}_{{\rm out},k}^{*} \} \nonumber \\ & \;\;\;\;\;\;\;\;\;\; - P_s \left|  { h}_{{\rm sr},k}  \right|^2 \cdot \left|a_k \right|^2 \Big )  + W^{(n)},   \label{eq:destructive_power}
\end{align} 
\begin{figure*}[!t]
% ensure that we have normalsize text
\normalsize
% Store the current equation number.
%\setcounter{MYtempeqncnt}{\value{equation}}
% Set the equation number to one less than the one
% desired for the first equation here.
% The value here will have to changed if equations
% are added or removed prior to the place these
% equations are referenced in the main text.
%\setcounter{equation}{MYtempeqncnt}
\begin{align}
\label{eqn_slnr}
{\rm SENR}_k^{(n)} &=  \frac{P_{{\rm desired},k}^{(n)}}{P_{{\rm destructive},k}^{(n)}} =  \frac{P_s  \cdot \left|a_k \right|^2 \left|  { h}_{{\rm sr},k}  { h}_{{\rm rd},k}^{(n)} \right|^2}  {\left|  { h}_{{\rm rd},k}^{(n)}  \right|^2  ( \frac{  \left(\eta_k+1 \right)  \left|a_k \right|^2  \left (P_s \left|  { h}_{{\rm sr},k} \right|^2 + M_k \right ) } {1 - \left|a_k \right|^2 \Big( \left|  { h}_{{\rm rr},k} \right|^2  \eta_k + (\gamma_k +1 ) \left|{ \delta}_{k} \right|^2  \Big)  } - P_s \left|  { h}_{{\rm sr},k}  \right|^2 \cdot \left|a_k \right|^2  )  + W^{(n)}}, \\
%& =  -1 + \frac{\tilde{a}_k\left(   \left( 1+  \gamma_k \right) \left|{ h}_{{\rm rd},k}^{(n)} \right|^2  \left (P_s \left|  { h}_{{\rm sr},k} \right|^2 + M_k \right ) - W^{(n)}  \left|{ h}_{{\rm rr},k} \right|^2 \eta_k    \right) + W^{(n)}} { \tilde{a}_k^2 \left(  \eta_k  P_s  \left|  { h}_{{\rm sr},k} { h}_{{\rm rr},k}  { h}_{{\rm rd},k}^{(n)} \right|^2   \right) + \tilde{a}_k \left( - W^{(n)}  \left|{ h}_{{\rm rr},k} \right|^2   \eta_k  -   P_s  \left|  { h}_{{\rm sr},k}  { h}_{{\rm rd},k}^{(n)} \right|^2   + \left( 1+  \gamma_k \right)  \left|{ h}_{{\rm rd},k}^{(n)} \right|^2 \left (P_s \left|  { h}_{{\rm sr},k} \right|^2 + M_k \right )   \right) +  W^{(n)} } \\
%& =  -1 + \frac{\tilde{a}_k c_1^{(n)} + W^{(n)}} { \tilde{a}_k^2 c_2^{(n)}  + \tilde{a}_k c_3^{(n)} +  W^{(n)} }, \;\;\;\;{\it where}\;\;\; \eta_k:= \gamma_k + \beta_k + \beta_k  \gamma_k, \;\; \tilde{a}_k := \left|a_k \right|^2.   
%\\  {\text{where}}\;\;\; \eta_k:&= \gamma_k + \beta_k + \beta_k  \gamma_k, \;\; b_{k}:= |  { \tilde{h} }_{{\rm rr},k} + \delta_k^{\star} |^2  \eta_k + (\gamma_k +1 ) |{ \delta}_{k}^{\star} |^2, \;\; \tilde{a}_k := \left|a_k \right|^2, \vspace{1mm} \nonumber \\
% Restore the current equation number.
%\setcounter{equation}{19}
% IEEE uses as a separator
%\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
% Store the current equation number.
%\setcounter{MYtempeqncnt}{\value{equation}}
% Set the equation number to one less than the one
% desired for the first equation here.
% The value here will have to changed if equations
% are added or removed prior to the place these
% equations are referenced in the main text.
%\setcounter{equation}{MYtempeqncnt}
\tilde{\rm SENR}_k :&= \underset{n \in \mathbb{S}_N,\;  \delta_k \in \mathcal{H}_k  }{ \rm min } \;\; {\rm SENR}_k^{(n)} = \underset{n \in \mathbb{S}_N  }{ \rm min } \;\; \left\{ \frac{P_s  \tilde{a}_k \left|  { h}_{{\rm sr},k}  \right|^2}  {  \frac{ \left( 1+  \eta_k \right) \tilde{a}_k \left (P_s \left|  { h}_{{\rm sr},k} \right|^2 + M_k \right ) } {1 - \tilde{a}_k  b_{k}  } - P_s \left|  { h}_{{\rm sr},k}  \right|^2 \cdot \tilde{a}_k  + {W^{(n)}}/{|{ h}_{{\rm rd},k}^{(n)}|^2 }} \right \}\vspace{1mm} \\
&= \frac{P_s \tilde{a}_k\left|  { h}_{{\rm sr},k}  \right|^2}  {  \frac{ \left( 1+  \eta_k \right) \tilde{a}_k \left (P_s \left|  { h}_{{\rm sr},k} \right|^2 + M_k \right ) } {1 - \tilde{a}_k  b_{k} } - P_s \left|  { h}_{{\rm sr},k}  \right|^2 \cdot \tilde{a}_k  + \ell_k }, \;\;  \\  {\text{where}}\;\;\; \eta_k:&= \gamma_k + \beta_k + \beta_k  \gamma_k, \;\; b_{k}:= |  { \tilde{h} }_{{\rm rr},k} + \delta_k^{\star} |^2  \eta_k + (\gamma_k +1 ) |{ \delta}_{k}^{\star} |^2, \;\;\ell_k := \underset{n \in \mathbb{S}_N  }{ \rm max }\;\; \left \{ {W^{(n)}}/{|{ h}_{{\rm rd},k}^{(n)}|^2 } \right \}, \;\; \tilde{a}_k := \left|a_k \right|^2. \vspace{1mm} \nonumber 
\end{align}
% Restore the current equation number.
%\setcounter{equation}{19}
% IEEE uses as a separator
\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
\vspace*{-0mm}
\end{figure*}where $P_{{\rm desired},k}^{(n)}, P_{{\rm destructive},k}^{(n)}$ respectively represent the power of the desired and destructive parts of the signal at $D_n$. 

{\it Lemma 1}: The worst-case $\delta_k \in \mathcal{H}_k$, denoted as $\delta_k^{\star}$, given the self-interference channel estimation $ {\tilde {h}}_{{\rm rr},k}$ is calculated as \mbox{$\delta_k^{\star} =  \frac{{\zeta_k }{\tilde {h}}_{{\rm rr},k}}{|{\tilde {h}}_{{\rm rr},k}|}$}.
\begin{proof}
It is apparent from (14) and (15) that the desired power is invariant to the choice of $\delta_k$. On the other hand, the value of $P_{{\rm destructive},k}^{(n)}$ is monotonic with respect to the transmit power from the relay. Hence, the worst-case $\delta_k$ is the one that minimizes the denominator in (13), or equivalently maximizes the term: $|  { \tilde{h} }_{{\rm rr},k} + \delta_k |^2  \eta_k + (\gamma_k +1 ) \left|{ \delta}_{k} \right|^2$. This results in the $\delta_k \in \mathcal{H}_k$ with maximum amplitude, and with similar phase as ${ \tilde{h} }_{{\rm rr},k}$, i.e., \mbox{$\delta_k^{\star} =  \frac{{\zeta_k }{\tilde {h}}_{{\rm rr},k}}{|{\tilde {h}}_{{\rm rr},k}|}$}. 
\end{proof}

The value of ${\rm SENR}_k^{(n)}$ is then formulated in (16) assuming $R_k$ is active with an arbitrary amplification coefficient ($a_k$), and self-interference channel estimation error $\delta_k$. As it is clear from (16), the phase of $a_k$ has no effect on the resulting $\rm SENR$. Hence we consider $\tilde{a}_k := \left|a_k \right|^2$ as our optimization parameter hereinafter. As it is formulated in (10), our goal is to maximize the worst-case link quality in the defined multicast system. The weakest link quality, denoted as $\tilde{\rm SENR}_k$ hereafter, can be hence formulated as a function of the selected relay and the corresponding amplification coefficient in (17) and consequently as (18). This is done by applying Lemma 1, and factoring the common channel coefficient ${ h}_{{\rm rd},k}^{(n)}$ from nominator and denominator of (16). It is important to note that while the value of $\tilde{\rm SENR}_k$ approaches zero for $\tilde{a}_k \rightarrow 0$ and $\tilde{a}_k \rightarrow  \tilde{a}_k^{\infty}$ ($\tilde{a}_k^{\infty} := \frac{1}{  b_{k}}$, see (18)), it remains positive and differentiable on all values in the range $(0, \tilde{a}_k^{\infty} )$. By incorporating (8), and observing the fact that $\mathcal{E} \{ {r}_{{\rm out},k}  {r}_{{\rm out},k}^{*} \}$ is monotonically increasing in $\tilde{a}_k$, the feasible region for $\tilde{a}_k$ is determined as $\tilde{a}_k \in [0, \tilde{a}_{k,{\rm max}}]$, where
\begin{align}
\tilde{a}_{k,{\rm max}}  :=  {P}_{k} \cdot \Big( ( 1 & +  \eta_k )  \left (P_s \left|  { h}_{{\rm sr},k} \right|^2 + M_k \right ) \nonumber \\ & + {P}_{k}  b_k     \Big)^{-1}, \;\;  0 \leq \tilde{a}_{k,{\rm max}} < \tilde{a}_k^{\infty}. 
\label{eq:limits}
\end{align}  
Note that the identity (18) holds for all feasible $a_k$ as $\tilde{\rm SENR}_k$ remains differentiable and continuous within the region $ 0 \leq \tilde{a}_{k} \leq \tilde{a}_{k,{\rm max}}$. The problem of maximizing the minimum link quality for a given selected relay can be hence formulated as 
%\left \{ -1 + \frac{\tilde{a}_k c_{k,1} + \ell_k} { \tilde{a}_k^2 c_{k,2}  + \tilde{a}_k c_{k,3} +  \ell_k } \right \}
\begin{align}
 \underset{\tilde{a}_{k} }{ \rm max }\;\; & (18)   , \nonumber \\
 {\rm s.t.} \;\;  & 0 \leq \tilde{a}_{k} \leq  \tilde{a}_{k, {\rm max}}.
\end{align}
By taking the derivative, the stationary points of the objective function can be achieved as 
\begin{align}
%r_1 = - \frac{c_2}{c_1} + \sqrt{ \left(\frac{c_2}{c_1}\right)^2 - \frac{c_2 d_2}{c_1 d_1} + \frac{d_3}{d_1}  } \nonumber \\
%r_2 = - \frac{c_2}{c_1} - \sqrt{ \left(\frac{c_2}{c_1}\right)^2 - \frac{c_2 d_2}{c_1 d_1} + \frac{d_3}{d_1}  }.
r_{k,1} = \frac{-1}{c_{k}-b_{k}} + \frac{\sqrt{{c_{k}}/{b_{k}}}}{\left| c_{k}-b_{k} \right|}, \nonumber \\
r_{k,2} = \frac{-1}{c_{k}-b_{k}} - \frac{\sqrt{{c_{k}}/{b_{k}}}}{\left| c_{k}-b_{k} \right|}, 
\end{align}
where $b_{k} := |  { \tilde{h} }_{{\rm rr},k} + \delta_k^{\star} |^2  \eta_k + (\gamma_k +1 ) \left|{ \delta}_{k}^{\star} \right|^2$ and $c_{k} := \frac{\left( 1+  \eta_k \right)  \left (P_s \left|  { h}_{{\rm sr},k} \right|^2 + M_k \right )} { \ell_k }\in \real^{+}$.
%where $b_{k,1} :=  \left|  { h}_{{\rm rr},k} \right|^2 \eta_k \in \real^{+}$ and $b_{k,2} := \frac{\left( 1+  \eta_k \right)  \left (P_s \left|  { h}_{{\rm sr},k} \right|^2 + M_k \right )} { \ell_k }\in \real^{+}$.

{\it Lemma 2}: The values of $r_{k,1},r_{k,2}$ are real for the defined system. Moreover, there exists exactly one extremum for $\tilde{\rm SENR}_k$ in the range $ \tilde{a}_k \in \left( 0, \tilde{a}_k^{\infty} \right) $. This extremum  is a maximum and obtained as the smallest non-negative value among $r_{k,1},r_{k,2}$. We name this value as $r_k^{\star}$ hereinafter.
\begin{proof}
See Appendix.
\end{proof}

The above Lemma leaves us with $\tilde{a}_k = r_k^\star$ as the SENR-maximizing point in the region $\left(0,  \tilde{a}_k^{\infty} \right)$. If $r_k^\star \leq \tilde{a}_{k,{\rm max}}$ (feasibility condition), then $r_k^\star$ represents the value of optimal $\tilde{a}_k$, see Fig. 3-a. On the other hand, since the $\tilde{\rm SENR}_k$ function has no other extrema in the aforementioned region, if $r_k^\star> \tilde{a}_{k,{\rm max}} $ then $\tilde{\rm SENR}_k$ is an increasing function of $\tilde{a}_k$ inside its feasible region. In such a case, the optimal $\tilde{a}_k$ is located on the boundary of the feasible region where $\tilde{a}_k$ holds the maximum feasible value, see Fig. 3-b. Hence we always achieve the optimal $\tilde{a}_k$ as
%where $\tilde{a}_k^{\star}, {a}_k^{\star}$ respectively represent the optimal values for $\tilde{a}_k$ and for the relay's amplification coefficient. The optimal minimum link quality, $\tilde{\rm SENR}_k$ can be consequently achieved via (18). It is worth mentioning that due to the single operation of the selected relay in this scenario, the phase of ${a}_k^{\star}$ does not affect the objective as it is clear from (17), (18). Following the same approach for all relays in the network, we achieve the optimal performance of end-to-end communication for the selection of each relay node. Obviously, the relay that offers the highest optimal ${\rm SENR}_k$ is the one to be selected according to (11). 
\begin{figure}[t]
\hspace{0.0cm} \subfigure[$r_k^{\star} \leq \tilde{a}_{{\rm max},k} $]{\includegraphics[angle = 0, width = 0.48\columnwidth]{drawing-2}}
\subfigure[$r_k^{\star} >\tilde{a}_{{\rm max},k} $]{\includegraphics[width = 0.48\columnwidth]{drawing-1}}
%\LoadClass[onecolumn]{article}
%\addtolength{\linewidth}{3.6in}
\caption{{\footnotesize{Possible situations of $r^{\star}$ considering the feasible region of $\tilde{a}_k$. The dark circle indicates the position of the optimum point. }} }
%\LoadClass[twocolumn]{article}
\vspace{-7pt}
\end{figure}
\begin{align}
\tilde{a}_k^{\star} = \min \left\{ r_k^{\star} , \tilde{a}_{k, {\rm max}} \right \}, \;\; {a}_k^{\star} = \sqrt{\tilde{a}_k^{\star}},
\end{align} 
where ${a}_k^{\star}$ represents the optimum relay amplification coefficient, assuming that $R_k$ is selected as the active relay. It is worth mentioning that due to the single operation of the relay node, the phase of ${a}_k^{\star}$ does not affect the objective as it is clear from (17), (18). The corresponding minimum link quality is then calculated via (18) and the relay node which offers the highest minimum link quality, will be the selected relay to forward the message from source. The performance of the defined FD relaying together with the obtained optimal design is demonstrated in Section VI with respect to different system parameters. 

\subsection{Computational Complexity}
It should be noted that while the updated solution is based on further knowledge of the loopback interference path, the final solution does not add a significant solution complexity in comparison to the traditional designs. From (22) and the formulation in (21) the overall required computation is calculated as  .. where ... . The aforementioned amount is very small, in comparison with the capability of the commonly used processors.  

As we have observed from above analysis, while the efficiency of the FD relaying can be increased due to simultaneous transmission and reception, the system behavior is different from the previous HD schemes due to the nature of the resulting residual interference. In the following we study the resulting system behavior for two extreme scenarios.
%%%%%%%Consequently, and the equivalency of (18) and (19) hold for all feasible values of $a_k$ where the power constraint (8) is fulfilled. It is worth mentioning that the resulting transmit power from each relay, and the consequent link quality (${\rm SENR}_k^{(n)}$) has the different structure compared to the classic scenario with HD relay nodes. This difference is evident considering the second order polynomial in the denominator of (20). This stems in the fact that in the FD scenario the transmit power affects the intensity of the residual self-interference in the receiver via the loopback path, see (1), (4), (6). As a result, the maximum amplification on the relay (corresponding to using the maximum relay individual power) in not necessarily optimal since increasing $|a_k|^2$ simultaneously increases the resulting error components at the relay's receiver end. In order to choose the best relay node and the corresponding $a_k$, we apply bi-section search on values of $t$ in (11), which turns our problem into a feasibility check for each value of $t$:
%%%%%%%\begin{align}
 %%%%%%%\underset{ }{ \rm find }\;\; &k,\tilde{a}_k,  \;\; k \in \mathbb{S}_K \nonumber \\
%%%%%%%{\rm s.t.} \;\; & {\rm SENR}_k^{(n)} \geq t, \;\; \forall \; n \in \mathbb{S}_N.
%%%%%%%\end{align}
%%%%%%%By incorporating (20) into (xxx) our problem can be reformulated as
%%%%%%%\begin{align}
 %%%%%%%\underset{ }{ \rm find }\;\; &k,\tilde{a}_k,  \;\; k \in \mathbb{S}_K \nonumber \\
%%%%%%%{\rm s.t.} \;\; & \tilde{a}_k \cdot \left(c_1^{(n)} - c_3^{(n)} \left( t+1 \right) \right) - \tilde{a}_k^2 \cdot \left( t+1 \right) c_2^{(n)} \nonumber \\ & \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; - t \cdot W^{(n)}  \geq 0, \;\; \forall \; n \in \mathbb{S}_N.
%%%%%%%\end{align} 
%%%%%%%As it is clear, the above problem is a combinatorial problem over $k$ with no direct optimal solution. Nevertheless, for a given relay node (fixed $k$) the problem turns into a convex feasibility problem which can be determined with certainty within a polynomial time \cite{xxx}. Therefore, we perform the feasibility check (22) by applying an exhaustive search over the available relay nodes ($R_k, \; \forall k \in \mathbb{S}_K$) and examine them individually as a convex feasibility check. It is clear that (22) is feasible if feasibility holds for any of the available relay nodes. The similar procedure for multiple steps of the bi-section search must be done until the required solution precision is achieved.
%%%%%%%
%%%%%%%While the proposed solution provides us with the optimal relay selection as well as the corresponding amplification coefficient, it is rather lengthy and requires several search steps. In the following we provide simplified solutions for the special setups.

    



   
%%%in the first step we observe from (18) that the value of ${\rm SENR}_k$ is invariant to $\angle{a_k}$. Hence we define $\tilde{a}_k := \left|a_k \right|^2$ and study the feasibility conditions for values of $\tilde{a}_k$. By incorporating (8) and (9) into (\ref{eq:tx_power}) we have:
%%%\begin{align}
%%%0 \leq \mathbb{E} & \{ {r}_{{\rm out},k}  {r}_{{\rm out},k}^{*} \} \leq \bar{P}_{\rm max}, \label{eq:tx_bounds}  
%%%\end{align}
%%%which consequently results in the following upper and lower bounds for $\tilde{a}_k$ 
%%%\begin{align}
%%%\tilde{a}_k &\geq 0, \nonumber \\
						%%%\tilde{a}_k &\leq   \bar{P}_{\rm max} \cdot \Bigg( \left( 1+  \gamma_k \right)  \left (P_s \left|  { h}_{{\rm sr},k} \right|^2 + M_k \right )  \nonumber \\ & \;\;\;\;\;\;\;\;+ \bar{P}_{\rm max}  \left|  { h}_{{\rm rr},k} \right|^2 \left( \gamma_k + \beta_k + \beta_k  \gamma_k  \right )     \Bigg)^{-1} =: \tilde{a}_k^{lim}, 
%%%\label{eq:limits}
%%%\end{align}
%%%where $\bar{P}_{\rm max}:= \min \left( P_{\rm tot}, P_{\rm max} \right)$. Note that the obtained upper bound for $\tilde{a}_k$ happens at the upper bound of the inequality in (\ref{eq:tx_bounds}), due to monotonic (increasing) nature of $\mathbb{E} & \{ {r}_{{\rm out},k}  {r}_{{\rm out},k}^{*} \}$ with respect to $\tilde{a}_k$ in the feasible domain. Now we study the behavior of ${{\rm SENR}_k}$ function for different values of $\tilde{a}_k$ to obtain the optimum point. As the first step we observe that both extremes of $\tilde{a}_k \rightarrow 0$ and $\tilde{a}_k \rightarrow  \tilde{a}_k^{\infty}$, $\tilde{a}_k^{\infty} := \frac{1}{  \left|  { h}_{{\rm rr},k} \right|^2 \left( \gamma_k + \beta_k + \beta_k  \gamma_k  \right ) }$, where the relay's transmit power approaches infinity, result in ${{\rm SENR}_k} = 0$. Furthermore,  due to the differentiable, positive and continuous nature of ${{\rm SENR}_k}$ between these two values, the maximum value of ${{\rm SENR}_k}$ occurs at an stationary point (a maximum) between these two values. Note that the ${{\rm SENR}_k}$-maximizing stationary point is not necessarily feasible. By formulating the ${{\rm SENR}_k}$ function into the following structure
%%%\begin{align}
%%%%\label{eqn_slnr}
%%%& {\rm SENR}_k = c_0 + \frac{c_1 \tilde{a}_k + c2 } {d_1 \tilde{a}_k^2 +  d_2 \tilde{a}_k +  d_3},
%%%\end{align}
%%%where $c_0,c_1,c_2,d_1,d_2,d_3 \in \real$ are directly replaced from (19), we find all stationary points of (19) as
%%%\begin{align}
%%%%\label{eqn_slnr}
%%%& \frac{\partial {\rm SENR}_k} {\partial \tilde{a}_k } =  0 \;\; \Leftrightarrow \nonumber \\
%%%& \tilde{a}_k ^2 + \tilde{a}_k \left( 2 \frac{c_2}{c_1} \right) + \left( - \frac{d_3}{d_1} +  \frac{d_2 c_2}{d_1 c_1} \right)=0.
%%%\end{align}
%%%The above equality is a classic second order polynomial function with two roots $r_1, r_2$ as 
%%%\begin{align}
%%%r_1 = - \frac{c_2}{c_1} + \sqrt{ \left(\frac{c_2}{c_1}\right)^2 - \frac{c_2 d_2}{c_1 d_1} + \frac{d_3}{d_1}  } \nonumber \\
%%%r_2 = - \frac{c_2}{c_1} - \sqrt{ \left(\frac{c_2}{c_1}\right)^2 - \frac{c_2 d_2}{c_1 d_1} + \frac{d_3}{d_1}  }.
%%%%r_1 = \frac{-1}{b_2-b_1} + \frac{\sqrt{{b_2}/{b_1}}}{\left| b_2-b_1 \right|} \nonumber \\
%%%%r_2 = \frac{-1}{b_2-b_1} - \frac{\sqrt{{b_2}/{b_1}}}{\left| b_2-b_1 \right|} 
%%%\end{align}
%%%
%%%{\it Lemma 1}: The values of $r_1,r_2$ are real for the defined system. Moreover, there exists exactly one extrema for ${\rm SENR}_k$ in the range $ \tilde{a}_k \in \left( 0, \tilde{a}_k^{\infty} \right) $. This extrema is a maximum and obtained as the smallest non-negative value among $r_1,r_2$. We name this value as $r^{\star}$ hereinafter.
%%%\begin{proof}
%%%See Appendix I.
%%%\end{proof}
%%%%
%%%%
%%%%where $b_1 =  \left|  { h}_{{\rm rr},k} \right|^2 \left( \gamma_k + \beta_k + \beta_k  \gamma_k  \right ) $ and $b_2 = \frac{\left( 1+  \gamma_k \right)  \left (P_s \left|  { h}_{{\rm sr},k} \right|^2 + M_k \right )}{W}$ and $b_1,b_2 \in \real^{+}$. 
%%%%Depending on the different system parameters (noise levels, channel situations, ...), $r^{\star}$ holds different values on the real axis. Nevertheless, according to Lemma 1, there always exists exactly one root (representing a maximum) which is located in the region $[0, \tilde{a}_k^{\infty} )$. This stems in the simple fact that while ${{\rm SENR}_k}$ remains differentiable, positive, and continuous in the aforementioned region, it returns to zero at two ends: $\tilde{a}_k \rightarrow 0$ and $\tilde{a}_k \rightarrow  \tilde{a}_k^{\infty}$. This indicates that ${{\rm SENR}_k}$ experiences an odd number of extremums in $[0, \tilde{a}_k^{\infty} )$. Since there can be no more than two extrema in the aforementioned region (due to second order polynomial), we conclude that exactly one of the obtained roots is representing a local maximum and is located in the region $[0, \tilde{a}_k^{\infty} )$. We name the aforementioned root as $r^\star$ hereinafter. The above argumentation leaves us with $\tilde{a}_k = r^\star$ as the SENR-maximizing value. If $r^\star \leq \tilde{a}_k^{ lim}$ (feasibility condition), then $r^\star$ represents the value of optimal $\tilde{a}_k$. On the other hand, since the ${{\rm SENR}_k}$ function has no other extrema in the defined region $\left[0,  \tilde{a}_k^{\infty} \right]$, if the extremum (maximum) point $\tilde{a}_k= r^\star$ is located outside of the feasible region (i.e., $r_1 > \tilde{a}_k^{ lim} $), then ${{\rm SENR}_k}$ is an increasing function of $\tilde{a}_k$ inside its feasible region. In such a case, the optimal $\tilde{a}_k$ is located on the boundary of the feasible region where $\tilde{a}_k$ holds the maximum feasible value. Hence we always achieve the optimal $\tilde{a}_k$ as
%%%\end{figure} 
%%%%\setlength{\intextsep}{10pt plus 200mm minus 200mm}
%%%\begin{figure}[t]
%%%\hspace{0.0cm} \subfloat[$r^{\star} > \tilde{a}_k^{lim} $]{\includegraphics[width = 0.5\columnwidth]{drawing-1}}
%%%\subfloat[$r^{\star} \leq \tilde{a}_k^{lim} $]{\includegraphics[angle = 0, width = 0.5\columnwidth]{drawing-2}}
%%%%\LoadClass[onecolumn]{article}
%%%%\addtolength{\linewidth}{3.6in}
%%%\caption{Possible situations of $r^{\star}$ considering the feasible region of $\tilde{a}_k$. The dark circle indicates the position of the optimum point.}
%%%%\LoadClass[twocolumn]{article}
%%%\end{figure}
%%%
%%%Depending on the different system parameters (noise levels, channel situations, ...), $r^{\star}$ holds different values on the real axis. Nevertheless, according to Lemma 1, there always exists exactly one root (representing a maximum) which is located in the region $\left(0, \tilde{a}_k^{\infty} \right)$. This leaves us with $\tilde{a}_k = r^\star$ as the SENR-maximizing point. If $r^\star \leq \tilde{a}_k^{ lim}$ (feasibility condition), then $r^\star$ represents the value of optimal $\tilde{a}_k$ (see Fig 1-a). On the other hand, since the ${{\rm SENR}_k}$ function has no other extrema in the defined region $\left(0,  \tilde{a}_k^{\infty} \right)$, if the extremum (maximum) point $\tilde{a}_k= r^\star$ is located outside of the feasible region (i.e., $r^{\star} > \tilde{a}_k^{ lim} $), then ${{\rm SENR}_k}$ is an increasing function of $\tilde{a}_k$ inside its feasible region  (see Fig 1-b). In such a case, the optimal $\tilde{a}_k$ is located on the boundary of the feasible region where $\tilde{a}_k$ holds the maximum feasible value. Hence we always achieve the optimal $\tilde{a}_k$ as
%%%\begin{align}
%%%\tilde{a}_k^{\star} = \min \left\{ r^{\star} ,  \tilde{a}_k^{ lim}\right \}, \;\; {a}_k^{\star} = \sqrt{\tilde{a}_k^{\star}},
%%%\end{align}
%%%where $\tilde{a}_k^{\star}, {a}_k^{\star}$ respectively represent the optimal values for $\tilde{a}_k$ and for the relay's amplification coefficient. The obtained optimal link quality (${\rm SENR}_k$) can be consequently achieved via (18). It is worth mentioning that due to the single operation of the selected relay in this scenario, the phase of ${a}_k^{\star}$ does not affect the objective as it is clear from (18), (19). Following the same approach for all relays in the network, we achieve the optimal performance of end-to-end communication for the selection of each relay node. Obviously, the relay that offers the highest optimal ${\rm SENR}_k$ is the one to be selected according to (11). 






==> main_PreviousOptimal.tex <==
In this section we define our optimization strategy and discuss the available solution to the defined problem.
\subsection {Optimization problem}
Our objective and system constraints are identical to those in \cite{RezaPassive1}. In order to achieve a good estimation of the observed
signal, the estimate must be as close as possible to the actual target signal. Hence the objective $V$ is chosen as the minimum mean squared error (MMSE) and is given by
\begin{align}
V := \mathcal{E} \{|\tilde{r} - r|^2\} = \sum_{k=1}^{K} |v_k|^2 \left( M_k |u_k|^2 |h_k|^2 + N_k  \right).
\end{align}
Furthermore, we limit our solution set to unbiased estimators which by considering (6) follow the identity 
\begin{align}
\sum_{k=1}^{K} c_k = 1, \;\;  c_k := g_{k}h_{k}u_{k}v_{k}.
\end{align}
By including the defined power constraints (3) and (4) we may now formulate our optimization problem as 
\begin{align}
\underset{u_k , v_k , \; k \in \mathbb{F}_K}{ \rm min }&  V  \nonumber  \\
{\rm s.t.} \;\;    &  \sum_{k \in \mathbb{F}_K} c_k= 1, 
\;\;\sum_{k \in \mathbb{F}_K} X_{k} \leq P_{\rm tot}, \nonumber \\
& X_{k} \leq P_{k}, \;\; \forall k \in \mathbb{F}_k.
\end{align} \vspace{-7mm}
%which defines our optimization strategy for the investigated system.
\subsection {Available solution}
The optimal solution to the above-mentioned problem is presented in \cite{RezaPassive1}, assuming real-valued amplification coefficients ($u_k \in \real^{+}$). For the detailed description of the solution please refer to \cite[Section III]{RezaPassive1}, equations (11-58). As it is been explained, the solution relies on the separation of the function of SNs into the nodes with zero allocated power (\emph{inactive} status, $X_k = 0$), the nodes with maximum allocated power (\emph{saturated}, $X_k = P_k$) and nodes with \emph{active} status ($0 < X_k < P_k$). While the presented procedure provides the optimal solution in closed form, the separation of nodes into correct status is only performed via an iterative search and examining the nodes combination. This process gets more complicated and occasionally leads to long searching periods as the number of the nodes increases. In the following we try to address this problem accordingly.

==> main_Quadratic_Approximation_Covariance_Shaping.tex <==
The proposed gradient-based optimization requires high iteration counts and imposes high computational complexity. In this Section, we propose an iterative method which is based on quadratic approximation of relay transmit covariance matrix, with respect to $\ma W$. In this way the resulting optimization problem can be cast as a separately convex (and not a jointly convex) optimization problem in each iteration. In each optimization iteration, ${\ma{Q}}^{(\ell)}$ is approximated as 
\begin{align} \label{eq_quadratic_approx}
{\ma{Q}}^{(\ell)} \approx {\ma W}^{(\ell)} \mathcal{R}\left({\ma{Q}^\star}^{(\ell -1)}\right) {{\ma W}^{(\ell)}}^H,
\end{align}
which indicates that the effect of distortion-loop is only updated between subsequent design iterations. The index $\ell$ represents the approximation iteration, and ${\ma{W}^\star}^{(\ell -1)},{\ma{Q}^\star}^{(\ell -1)}$ are the obtained ${\ma{W}}$ and ${\ma{Q}}$ in the $\ell-1$-th optimization step.\footnote{The value of ${\ma{Q}^\star}^{(0)}$ can be initialized similar to Algorithm 1.} It is worth mentioning, that the defined approximation (\ref{eq_quadratic_approx}) becomes more accurate as the distortion coefficients, i.e, $\beta$ and $\gamma$, become smaller and the distortion components in (\ref{eq_loop_U_out_R}) become negligible. Applying $P_{\rm s}^{\star} = P_{\text {s,max}}$ and exploiting the fact that the ratio $\frac{P_{\text{desired}}}{P_{\text{error}}}$ is strictly monotonic with respect to $\epsilon := \frac{P_{\text{desired}}}{P_{\text{tot}}}$, the optimization problem (\ref{eq_loop_optimization_problem_a})-(\ref{eq_loop_optimization_problem_b}) can be approximated in iteration $\ell$ as  
\begin{subequations} 
\begin{align} 
\underset{{\ma{z}}^{(\ell)}, {\ma{W}}^{(\ell)},{\ma{Q}}^{(\ell)},\epsilon \in \real_+}{\text{max}} \;\;\; & \epsilon \label{eq_quad_op1_a} \\
\text {s.t.} \;\;\;\;\;\;\; & \text{tr}\left( {\ma{Q}}^{(\ell)} \right) \leq \tilde{P}_{\rm{r,max}},  \;\; \text{and (\ref{eq_quadratic_approx})}, \label{eq_quad_op1_b}
\end{align}
\end{subequations}  
where the last constraint enforces the covariance approximation (\ref{eq_quadratic_approx}), as well as the positive semi-definiteness constraint for the relay undistorted transmit covariance. A feasibility check, corresponding to the ratio $\epsilon$ in the $\ell$-th approximation iteration can be hence written as
\begin{subequations} 
\begin{align} 
{\text{find}} \;\;\; & {{\ma{z}}^{(\ell)}, {\ma{W}}^{(\ell)}, {\ma{Q}}^{(\ell)} , t^{(\ell)} }   \label{eq_quad_op2_a} \\
\text {s.t.} \;\;\; & {P_{\rm{tot}}} \leq t^{(\ell)}, \;\; {P_{\rm{desired}}} \geq t^{(\ell)}\epsilon,   \label{eq_quad_op2_b} 
 \\ & \text{tr}\left( {\ma{Q}}^{(\ell)} \right) \leq P_{\rm{r,max}}, \;\; t^{(\ell)} >0, \;\; \text{and (\ref{eq_quadratic_approx})},   \label{eq_quad_op2_c}
\end{align}
\end{subequations}  
or equivalently as 
\begin{subequations} 
\begin{align} 
\underset{\small{{\ma{z}}^{(\ell)}, {\ma{W}}^{(\ell)},{\ma{Q}}^{(\ell)},t^{(\ell)}}}{\text{max}} \;\;\; &  {P_{\rm{desired}}} - t^{(\ell)}\epsilon   \label{eq_quad_op3_a} \\
\text {s.t.} \;\;\;\;\;\;\;\;\; & {P_{\rm{tot}}} \leq t^{(\ell)}, \;\;  \text{ and (\ref{eq_quad_op2_c})},    \label{eq_quad_op3_b}
\end{align} 
\end{subequations} 
where a value $\epsilon$ with a corresponding ${\ma{z}}^{(\ell)}, {\ma{W}}^{(\ell)}, {\ma{Q}}^{(\ell)} , t^{(\ell)} $ is feasible iff the maximized objective in (\ref{eq_quad_op3_a}) is not negative. Note that for each step of the covariance approximation in (\ref{eq_quadratic_approx}), the maximization (\ref{eq_quad_op1_a})-(\ref{eq_quad_op1_b}) should be solved. Hence, for a given $\ell$, we look for the maximum value of $\epsilon$ for which the feasibility holds. The defined feasibility check (\ref{eq_quad_op3_a})-(\ref{eq_quad_op3_b}) is re-formulated as
\begin{subequations} 
\begin{align} 
\underset{{\ma{z}}^{(\ell)}, {\ma{W}}^{(\ell)}, t^{(\ell)} }{\text{max}} \;\;\; &  {\ma{w}^{(\ell)}}^H {\ma{C}}^{(\ell)}{\ma{w}^{(\ell)}}  - t^{(\ell)} \epsilon  \label{eq_quad_op4_a} \\
\text {s.t.} \;\;\;\;\;\;\;\;\; & {{\ma{z}}^{(\ell)}}^H \Big(  {\ma{H}}_{\text {rd}}{\ma W}^{(\ell)} \mathcal{R}\left({\ma{Q}^\star}^{(\ell -1)}\right) {{\ma W}^{(\ell)}}^H  {{\ma{H}}_{\text {rd}}}^H \nonumber \\ & \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; + \sigma_{\text{nd}}^2 \ma{I}_{M_{\text{d}}} \Big) {{\ma{z}}^{(\ell)}} \leq t^{(\ell)},  \label{eq_quad_op4_b}\\ &  \text{tr}\left( {\ma W}^{(\ell)} \mathcal{R}\left({\ma{Q}^\star}^{(\ell -1)}\right) {{\ma W}^{(\ell)}}^H\right)  \leq P_{\rm{r,max}},   \label{eq_quad_op4_c}
\end{align} 
\end{subequations}  
where ${\ma{w}}^{(\ell)} := \text{vec} \left( {\ma{W}}^{(\ell)} \right)$, and 
{{\begin{align} 
{\ma{C}}^{(\ell)} := P_{\text {s,max}}\Big[{\ma{h}}_{\text {sr}}^T \otimes \left({\ma{z}^{(\ell)}}^H {\ma{H}}_{\text {rd}}\right)\Big]^H \Big[{\ma{h}}_{\text {sr}}^T \otimes \left({\ma{z}^{(\ell)}}^H {\ma{H}}_{\text {rd}}\right)\Big].
\end{align}}}Our approach is to provide a maximization process for (\ref{eq_quad_op4_a})-(\ref{eq_quad_op4_c}) together with an iterative update of $\epsilon$, until a joint stable point for $\epsilon$ and the optimization variables ${\ma{z}}^{(\ell)}, {\ma{W}}^{(\ell)}, t^{(\ell)}$ is achieved. Unfortunately, (\ref{eq_quad_op4_a})-(\ref{eq_quad_op4_c}) is not a convex optimization problem and also can not be solved in a closed form. The following Lemma will be consequently used to provide a multi-convex solution for (\ref{eq_quad_op4_a})-(\ref{eq_quad_op4_c}). 

\textit{Lemma 1.} The maximization of ${\ma{w}}^H {\ma{C}}{\ma{w}}$ over ${\ma{w}}$, is equivalent to 
\begin{align} 
\underset{{\ma{w}},{\ma{q}} }{\text{max}} \;\;\; & {\ma{w}}^H {\ma{C}}{\ma{q}} + {\ma{q}}^H {\ma{C}}{\ma{w}} - {\ma{q}}^H {\ma{C}}{\ma{q}}. \label{eq_lemma}
\end{align}
where ${\ma{q}}$ is a complex vector with the same size as ${\ma{w}}$ and ${\ma{C}} \succeq 0$.  
\begin{proof}
The maximization of (\ref{eq_lemma}) over $\ma{q}$ is an unconstrained convex problem. By equalizing the derivative to zero we obtain an optimal $\ma{q}$ as $\ma{q}^{\star} = \ma{w}$. This consequently equalizes the objective in (\ref{eq_lemma}) to ${\ma{w}}^H {\ma{C}}{\ma{w}}$. 
\end{proof}
By applying Lemma~1 and the results of the well-known Schur's complement \cite{BV:04}, (\ref{eq_quad_op4_a})-(\ref{eq_quad_op4_c}) is formulated as 
\begin{subequations} 
{\small{\begin{align} 
\underset{{{  		\begin{array}{c} 
		 {\ma{z}}^{(\ell)}, {\ma{w}}^{(\ell)}, \\
		{\ma{q}}^{(\ell)}, t^{(\ell)}  \\
		\end{array}  } }} {\text{max}} \;\;\; &  \Big\{ {\ma{w}^{(\ell)}}^H {\ma{C}}^{(\ell)}{\ma{q}^{(\ell)}} + {\ma{q}^{(\ell)}}^H {\ma{C}}^{(\ell)}{\ma{w}^{(\ell)}} \nonumber \\[-8mm]  & \;\;\;\;\;\;\;\;\;\;\;\; - {\ma{q}^{(\ell)}}^H {\ma{C}}^{(\ell)}{\ma{q}^{(\ell)}} - t^{(\ell)}\epsilon  \Big\} \label{eq_quad_op5_a} \\
\text {s.t.} \;\;\;\;\;\;\;\;\;\;\; & \left[
		\begin{array}{cc} 
		t^{(\ell)} - \sigma_{\text{nd}}^2 \|{{\ma{z}}^{(\ell)}}\|_2^2 	&  {{\ma{z}}^{(\ell)}}^H {\ma{H}}_{\text {rd}}{\ma W}^{(\ell)}   \\
		{{\ma W}^{(\ell)}}^H  {{\ma{H}}_{\text {rd}}}^H {{\ma{z}}^{(\ell)}} & \mathcal{R}\left({\ma{Q}^\star}^{(\ell -1)}\right)^{-1} \\
		\end{array} 
		\right] \succeq 0, \label{eq_quad_op5_b}  \\
		& \left[
		\begin{array}{cc} 
		P_{\rm{r,max}} 	&  {{\ma w}^{(\ell)}}^H   \\
		{{\ma w}^{(\ell)}}  & \tilde{\mathcal{R}}\left({\ma{Q}^\star}^{(\ell -1)}\right)^{-1} \\
		\end{array} 
		\right] \succeq 0, \;\; t^{(\ell)} >0,  \label{eq_quad_op5_c}
\end{align}}} 
\end{subequations}  
where 
\begin{align} 
\tilde{\mathcal{R}}:= \Big( {{\mathcal{R}}^{\frac{1}{2}}}^T \otimes \ma{I}_{{M_{\rm r}}} \Big)^H \Big( {{\mathcal{R}}^{\frac{1}{2}}}^T \otimes \ma{I}_{{M_{\rm r}}} \Big).
\end{align}
Note that (\ref{eq_quad_op5_a})-(\ref{eq_quad_op5_c}) is not a jointly convex optimization problem. Nevertheless it is jointly convex over ${\ma{w}}^{(\ell)},t^{(\ell)}$ or ${\ma{q}}^{(\ell)},t^{(\ell)}$, in each case if the other two variables are kept constant. Furthermore, for any value of ${\ma{w}}^{(\ell)}$, the optimal ${{\ma{z}}^{(\ell)}}$ can be calculated from (\ref{eq_GP_z}). This facilitates an iterative optimization for (\ref{eq_quad_op5_a})-(\ref{eq_quad_op5_c}) where in each step the problem is reduced to a convex problem. After each optimization step, the value of $\epsilon$ will be updated to equalize the objective (\ref{eq_quad_op5_a}) to zero:
\begin{align} 
\epsilon \leftarrow \frac{{\ma{w}^{(\ell)}}^H {\ma{C}}^{(\ell)}{\ma{q}^{(\ell)}} + {\ma{q}^{(\ell)}}^H {\ma{C}}^{(\ell)}{\ma{w}^{(\ell)}}  - {\ma{q}^{(\ell)}}^H {\ma{C}}^{(\ell)}{\ma{q}^{(\ell)}} }{t^{(\ell)}}. \label{eq_quad_epsilon}
\end{align}
The above update results in a feasible $\epsilon$ for the corresponding values of ${\ma{w}}^{(\ell)},{\ma{z}}^{(\ell)},t^{(\ell)}$, see (\ref{eq_quad_op3_a}) in connection to Lemma~1. The aforementioned process, i.e., the iterative optimization of (\ref{eq_quad_op5_a})-(\ref{eq_quad_op5_c}) and the update for $\epsilon$ will be continued until a stable point is achieved. The detailed optimization steps for this method is defined in Algorithm~2.
\subsection{Convergence and Algorithm Description}
Due to the described separate convexity of (\ref{eq_quad_op5_a})-(\ref{eq_quad_op5_c}), the objective value (\ref{eq_quad_op5_a}) will be necessarily increased after each optimization step. As the result, each update of $\epsilon$ results in a necessary increase. The aforementioned monotonicity results in a necessary convergence in the choice of ${\ma{w}}^{(\ell)},{\ma{z}}^{(\ell)},t^{(\ell)}$, which leads to a local optimum solution. Nevertheless, the resulting stable point is not necessarily a global optimum. If necessary, multiple initializations for $t^{(\ell)}$ and ${{\ma{z}}^{(\ell)}}$ can be used for solving (\ref{eq_quad_op5_a})-(\ref{eq_quad_op5_c}) to ensure, with higher confidence, the global optimality. The resulting solution for (\ref{eq_quad_op5_a})-(\ref{eq_quad_op5_c}), and hence for (\ref{eq_quad_op1_a})-(\ref{eq_quad_op1_c}), will be used as the approximation points in (\ref{eq_quadratic_approx}) in the next approximation iteration, i.e., $\ell + 1$. Similar process will be repeated until a stable point is achieved over multiple approximation iterations, or until a certain iteration count is expired.       





\begin{algorithm}[H]
 \small{	\begin{algorithmic}[1]
  %\SetAlgoLined
\State{$\ell \leftarrow 0$}
\State{$P_{\rm s} \leftarrow  P_{\rm{s,max}}  $}
\State{$\ma{Q}^{(0)} \leftarrow  \text{random init., see (\ref{eq_loop_optimization_problem_b})} $}
\State{$\ma{W}^{(0)} \leftarrow  {\ma{Q}^{(0)}}^{\frac{1}{2}} \mathcal{R}^{\frac{-1}{2}}\left(\ma{Q}^{(0)}\right), \text{ see (\ref{eq_GP_proj_W})-(\ref{eq_loop_U_out_R})}  $}
\Repeat 
\State{$\ell \leftarrow \ell + 1 $}
\Repeat

\State{$\ma{W}^{(\ell)},\ma{t}^{(\ell)} \leftarrow \text{solve (\ref{eq_quad_op5_a})-(\ref{eq_quad_op5_c})over } \ma{W}^{(\ell)},\ma{t}^{(\ell)},$}
\State{$\ma{q}^{(\ell)},\ma{t}^{(\ell)} \leftarrow \text{solve (\ref{eq_quad_op5_a})-(\ref{eq_quad_op5_c}) over } \ma{q}^{(\ell)},\ma{t}^{(\ell)},$}
\State{$\ma{z}^{(\ell)} \leftarrow \text{see  (\ref{eq_GP_z})},$}
\State{New $\epsilon \leftarrow \text{update } \epsilon, \text{see (\ref{eq_quad_epsilon})} $}
%\If{ \text{stable SINR value}}
%\State{break} 
%\EndIf
\Until {$|\text{New} \, \epsilon \;\; - \epsilon|\geq \theta_1$ }
\Until {$\| {\ma{W}^\star}^{(\ell)} - {\ma{W}^\star}^{(\ell-1)} \|_{\text{fro}}^2 \geq \theta_2$}
\State{\Return{$\ma{W}^{(\ell)},\ma{Q}^{(\ell)},\ma{z}^{(\ell)},\epsilon$} }
%%%
%%%project W
%%%choose z
%%%if stable break
%%%end
%%%end
 %%%%\Procedure{iterative optimization}{}
  %%%%\State {obtain  $\hat{J}_{k}\left(0 \right),\hat{J}_{k} \left( X_k^{\star} \right), \; k \in \mathbb{F}_{ K}$ \rhd see (22)} \\
%%%\State{\mbox{\small{$b_1\leq \cdots\leq b_{2K} \; \leftarrow \; \text{sort} \left\{ {J_k^{'}(0)}/ {\eta_k{'}},\; {J_k^{'}(X_{k,{\rm max}})}/ {\eta_k{'}}, \; \forall k \in \mathbb{F}_{ K} \right\}$}}} 
%%%
 %%%\hfill  $\rhd \; {\rm see} \; (16)$ 
%%%%\State{P_tot \leftarrow \min\{ \sum_{k \in \mathbb{K}_{\rm sat} } \}}
%%%\State{${ i_{\rm  min}} \leftarrow 1, \;\; {i_{\rm  max}} \leftarrow 2K+1$}
%%%
%%%\Repeat 
%%%
%%%\State{$i \leftarrow \lfloor \frac{{ i_{\rm min}} + { i_{\rm max}}}{2} \rfloor$}
%%%
%%%\State{$ \mathbb{K}_{\rm 0} \leftarrow \left\{k \in \mathbb{F}_{ K} \mid b_i \geq  {J_k^{'}(0)}/ {\eta_k{'}} \right\} \hfill  \rhd \; {\rm see \; (17a)}$}
%%%
%%%\State{$ \mathbb{K}_{\rm sat} \leftarrow \left\{k \in \mathbb{F}_{ K} \mid b_{i+1} \leq  {J_k^{'}(X_{k,{\rm max}})}/ {\eta_k{'}} \right\} \hfill  \rhd \; {\rm see \; (17b)}$}
%%%
%%%\State{$ \mathbb{K} \leftarrow  \mathbb{F}_{ K} \setminus \left( \mathbb{K}_{\rm sat} \cup \mathbb{K}_{ 0} \right) $} 
%%%
%%%\State {$ \tilde{V}_{\rm remain} \leftarrow V_{\rm max}^{-1} - \sum_{k \in \mathbb{K}_{\rm sat}  }  {J_k(X_{k,{\rm max}})} $}
%%%
%%%\If{ $\mathbb{K} = \emptyset $} 
          %%%\If{$\tilde{V}_{\rm remain} =0 $} \State{$\textbf{break}$} 
					%%%\ElsIf{$\tilde{V}_{\rm remain} <0$} \State{$i_{\rm  min} \leftarrow i$} 
           %%%\ElsIf{$\tilde{V}_{\rm remain} >0$} \State{$i_{\rm  max} \leftarrow i$} \EndIf
%%%\Else
%%%
%%%\State{{$\lambda^{\star} \leftarrow  \left( \frac    { \sum_{k \in \mathbb{K}} \alpha_k\beta_k \sqrt{{\eta_k{'}}} } {  V_{\rm max}^{-1} \hspace{-1pt}- \hspace{-5pt}\sum\limits_{k \in \mathbb{K}_{\rm sat}} \hspace{-7pt} J_k(X_{k,{\rm max}})\hspace{-1pt} -\hspace{-2pt} \sum\limits_{k \in \mathbb{K}} \hspace{-4pt} \alpha_k^2   }\right)^2 \hfill  \rhd \; {\rm see} \; (22)$ }}
%%%
%%%\If{$\frac{1}{\lambda^{\star}} > b_{i+1}\;\textbf{or}\; V_{\rm max}^{-1}  < \sum_{k \in \mathbb{K}_{\rm sat}}  {J_k(X_{k,{\rm max}})}$} 
%%%\State{$i_{\rm  min} \leftarrow i$} 
%%%\Else \State{$i_{\rm  max} \leftarrow i$} 
%%%\EndIf
%%%\EndIf
%%%
%%%\Until {$\left(\frac{1}{\lambda^{\star}} > b_i \; \textbf{and} \; \frac{1}{\lambda^{\star}} < b_{i+1} \right)$  }
%%%
%%%\State{$X_k \leftarrow \; \alpha_k\beta_k \sqrt{\frac{\lambda^{\star}} {{\eta_k{'}}}}  - \beta_k^2, \; k \in \mathbb{K} \hfill  \rhd \; {\rm see} \; (21) $}
%%%
%%%
%%%%\State{\Return{$\left( \mathbb{K}_{\rm sat}, \mathbb{F}_{0}, X_k k \in \mathbb{F}_{K} \right)$} }
%%%\State{\Return{$\left(\mathbb{K}_{\rm sat}, \mathbb{K}_{0}, \; X_k, k \in \mathbb{K}  \right)$} }
 %\EndProcedure
  \end{algorithmic} }
 \caption{\small{Iterative Covariance Shaping algorithm via Quadratic Approximation. $\theta_1,\theta_2 \in \real_+$ respectively define the stability conditions. } }

\end{algorithm} 

==> main_SubOpt_AF.tex <==
In this part we investigate the behavior of the optimal design for different special cases. In particular, we investigate the case where the distortion components at the FD relay nodes are negligible due to the sufficient precision of the hardware components, as well as the case where the noise power is ignorable at the destination nodes. The aforementioned scenarios respectively correspond to the FD system with high dynamic range and the system which operates in a high SNR region.
\subsection{Special case: $W^{(n)} \rightarrow 0, \; M_k \rightarrow 0 $}
This scenario corresponds to the case where the receiver thermal noise floor is ignorable compared to the incoming signal power at the receiver ends. By applying the above assumptions to (16) we formulate the corresponding $\rm SENR$ values as
\begin{align}
\underset{n \in \mathbb{S}_N  }{ \rm min }\;\;{\rm SENR}_k^{(n)} & = \frac{P_s  \cdot \left|a_k \right|^2 \left|  { h}_{{\rm sr},k}  \right|^2}  {  \frac{ \left( 1+  \eta_k \right) \left|a_k \right|^2  P_s \left|  { h}_{{\rm sr},k} \right|^2  } {1 - \left|a_k \right|^2   b_{k} } - P_s \left|  { h}_{{\rm sr},k}  \right|^2 \cdot \left|a_k \right|^2 } \nonumber \\
& = \frac{1}  {  \frac{ \left( 1+  \eta_k \right)  } {1 - \left|a_k \right|^2 b_{k}   } - 1 }.
\end{align}  
As it is clear, (23) is monotonically decreasing in $\tilde{a}_{k}$ in the feasible range. Hence as the value of $\tilde{a}_{k}$ approaches zero, the resulting  ${\rm SENR}_k^{(n)}$ corresponding to the weakest link approaches to $\frac{1}{\eta_k} = \left( \beta_k + \gamma_k + \beta_k \gamma_k \right)^{-1} $ as the upper bound to the optimal achievable minimum SENR. Nevertheless, this value may never be achieved in practice as the presence of any noise components results in zero SENR at the destination nodes for an extremely small choice of $\tilde{a}_{k}$. We recall that in the current scenario, the performance is limited only by the effects of limited system dynamic range (i.e. inaccuracies in ADC, DAC, ...) and limited digital domain estimation accuracy, excluding the effect of the thermal noise on the receiver front end.

\subsection {Special case: $ \beta_k, \gamma_k, \zeta_k \rightarrow 0$}   
This case corresponds to a FD system with accurate function of the involved transceiver components. In practice this can be approached by using more accurate elements in the system (e.g., ADC module with higher resolution) and effective passive isolation between Tx and Rx which alleviates the effects of distortion components. In this scenario the $\rm SENR$ formulation is significantly simplified and second order terms at the denominator of (18) disappear: 
\begin{align}
\label{eqn_slnr}
&\underset{n \in \mathbb{S}_N ,\;  \delta_k \in \mathcal{H}_k }{ \rm min }\;\;  {\rm SENR}_k^{(n)} =  \frac{P_s  \cdot \tilde{a}_k \left|  { h}_{{\rm sr},k}   \right|^2}  {  {  \tilde{a}_k  M_k  }     + \ell_k }, 
\end{align}
which is a monotonically increasing function with respect to $\tilde{a}_k$ and results in the maximum amplification at the relay in the optimum point. We should note that this is the similar problem structure to the equivalent HD system, where the self-interference does not exist at the relays \cite{MSKS:2012}. Nevertheless, higher efficiency is achieved due to FD operation at the relay nodes, which results in doubling the achievable communication rate. 

\subsection {System behavior interpretation}
As we have observed, the two aforementioned extreme scenarios lead to opposite optimal designs in terms of transmit power. In the first case, where system performance is dominated by the distortion components, the system tends to consume a very small power at the relay node. Furthermore, increasing the transmit power from the source doesn’t affect the resulting performance bound, which is obtained as $\frac{1}{\eta_k}$. On the other hand, the maximum relay power is used in the second case where distortion components are ignored and system performance is limited by noise. In this case, increasing $P_s$ results in the higher link quality. As it is partly described in Section II, the opposite behavior of the aforementioned cases stems from the fact that the variance of the distortion components, unlike the noise components, are dependent on the Tx and Rx signal power at the corresponding chain, see Fig.~2. Unlike the HD scenario where the maximum transmit power is used at optimality, this observation reveals the significance of power optimization at the FD relays, prior to relay selection. 

==> main_appendic_min_Eucklidean_Dist.tex <==
 

==> main_conclusion.tex <==
%In a simplistic view, the classic signal-loop for systems with feedback can be ignored for a FD relay, as the self-interference signal can be estimated and canceled. 
It is already known that for a system with FD operation, the performance can be degraded due to the residual self-interference, remaining from the self-interference cancellation process. In this work, we have shown that a FD and non-regenerative (AF) relaying system suffers additionally from a distortion loop, connecting the power of the transmit signal to the residual interference components: As the transmit power from the relay increases, the resulting inaccuracies increase both in Tx and Rx chains. These inaccuracies remain as residual interference components, which are then amplified in the relaying process and further increase the transmit power. In this work, we have analytically studied the effects of this power loop and particularly observed how this deviates the optimal design structure from the traditional designs, in which the effects of this loop have been neglected. The simulation results in Section V, as well as the analysis in Section IV, reinforce the importance of the proposed approach.  
%In a simplistic view, the classic signal-loop for systems with feedback can be avoided for a FD-AF relay, as the self-interference signal can be estimated and suppressed. In reality we observe a distortion loop, connecting the intensity of the desired and undesired signals: as the transmit power from the relay increases, the resulting inaccuracies increase both in Tx and Rx chains and remain as the residual self-interference. These residual components are then amplified and further increase the transmit power. In this work, we have analytically studied the effects of this loop and particularly observed how this deviates the optimal design structure from the previous designs, where this loop is avoided via simplifying assumptions. At the end we conclude the importance of \emph{joint power optimization and relay selection}, for the network of FD-AF relays as it is apparent from analysis in Section IV and numerical simulation, specially at high SNR region.

==> main_sysmodel_old.tex <==
\begin{table}[!t]
  \renewcommand{\arraystretch}{1.1}
  \caption{List of the used symbols in the defined system}\label{tab:notation}
  \centering
  \begin{tabular}[t]{c|l}
%  \firsthline
   Notation & Description \\
   \hline
	 $s, P_s$              &  transmit signal from the source and its power\\
   $\ma{h}_{{\rm sr}}$              & channel coefficient vector for the source-relay path\\
	 $\ma{H}_{{\rm rd}}$         & channel coefficient matrix for the relay-destination path\\
	 $\ma{ H}_{{\rm rr}}$              & channel coefficient matrix for the self-interference path\\
	 $ \ma{Q}$            &  relay transmit covariance matrix\\
   $ \ma{W}$            &  relay amplification matrix\\
	 $\ma z$              &  linear receive filter\\
	 %%${\tilde{ h} }_{{\rm rr},k} $              & estimated self-interference channel coefficient\\
	 %$\delta_k$              & self-interference channel estimation error\\	
   %$\mathcal{H}_k$              & set of all feasible self-interference channel estimation errors\\	
	 %$\delta_k^{\star}$              & the worst-case feasible $\delta_k \in \mathcal{H}_k$\\	
	 $\gamma, \beta$              & ratios representing Tx and Rx chain's dynamic range\\
	 %$\beta_k$              & ratio representing Rx chain's dynamic range\\
	 $\ma{n}_{\rm{nr}}, \sigma_{\rm{nr}}^2 $              & noise at the relay and its variance \\
	 $\ma{n}_{\rm{d}}, \sigma_{\rm{nd}}^2 $              & noise at the destination and its variance \\
   %$w^{(n)},W^{(n)}$      &  the additive white noise at $D_n$ and its variance \\
   $\ma{e}_{{\rm in}},\ma{e}_{{\rm out}}$      & error signals originating from Rx and Tx chains\\
	 $\ma{ r}_{{\rm in}},\ma{ r}_{{\rm out}}$          &  input and output signals at the relay\\
   $\ma{ u}_{{\rm in}},\ma{ u}_{{\rm out}}$          &  non-distorted received and transmit signals at the relay\\
   $ P_{\rm{r,max}}$            &  maximum allowed relay transmit power\\
	 $ P_{\rm{s,max}}$              &  maximum allowed source transmit power\\
   %${\mathbb K}$      & index set of all selected (active) relay nodes;\\	
   %${y}^{(n)}$      &  delivered signal at $D_n$\\	
  %\lasthline
  \end{tabular}\vspace{-3mm} 
\end{table}
\begin{figure*}[!t]
% ensure that we have normalsize text
\normalsize
        \includegraphics[angle=0,width=2.05\columnwidth]{model7.pdf}
% Restore the current equation number.
%\setcounter{equation}{19}
% IEEE uses as a separator
\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
    \caption{{\footnotesize{The interaction of different signal components in an amplify-and-forward FD MIMO relay node. The loopback-self interference affects the residual interference intensity. The red signal represents the self-interference signal while the green signal represents the suppressible (estimated) interference part. The bold arrows represent the vector signals while the dashed arrows represent the scalars. See Table~I for symbol descriptions.}} }
\vspace{-0pt}
\end{figure*}

We investigate a scenario where a single-antenna HD source communicates with a HD destination node with $M_{\text{d}}$ antennas, with a help of a FD relay. The relay is assumed to have $M_{\text{r}}$ transmit and receive antennas, and operate in AF mode. The channel between the source and the relay and between relay to destination are denoted as $\ma{h}_{\text{sr}} \in \compl^{M_{\text{r}}}$ and $\ma{H}_{\text{rd}} \in \compl^{M_{\text{d}} \times M_{\text{r}}}$, respectively. The self-interference channel, which is the channel between the relay's transmit and receive ends is denoted as $\ma{H}_{\text{rr}} \in \compl^{M_{\text{r}} \times M_{\text{r}}}$. All channels are following the block-flat fading model and the path between source to destination is assumed ignorable in this work.
 
\subsection {Source-to-Relay Communication}

The relay continuously receives and amplifies the received signal from the source, while tackling with the loopback self-interference signal from its own transmitter front-end, see Fig. 1. This is done by utilizing the known self-interference cancellation techniques, e.g., \cite{Bharadia:14,BMK:13}. The received signal at the relay is 
\begin{align} \label{eq_model_r_in}
\ma{ r}_{{\rm in}} =   \underbrace{\ma{ h}_{{\rm sr}}  \sqrt{P_s}s + \ma{H}_{{\rm rr}} \ma{r}_{{\rm out}} + \ma{n}_{\rm r} }_{=: \ma{u}_{\rm{in}}} +  \ma{e}_{{\rm in}}, \;\; P_{\rm s} \leq P_{\rm {s,max}}, 
%& \underbrace{ { h}_{{\rm sr},k} \cdot s + {\tilde{h}}_{{\rm rr},k} \cdot {r}_{{\rm out},k} + {\delta}_{k} \cdot {r}_{{\rm out},k} + {m}_{k} }_{ =: { u}_{{\rm in},k} } +  {e}_{{\rm in},k}, 
%&{\ma r}_{\rm y}  = \underbrace{ {\ma h}_{\rm sr} \cdot s + {\ma H}_{\rm rr} \cdot {\ma r}_{\rm x}  + \ma{n}_{\rm r} }_{{\ma u}_1 }  +  \ma{e}_{1} ,
\end{align}
where $\ma{r}_{{\rm in}}, \ma{r}_{{\rm out}} \in \compl^{M_{\rm r}}$ respectively represent the received and transmitted signal from the relay and $\ma{n}_{\rm{r}} \sim \mathcal{CN} \{ \ma{0}, \sigma_{\rm{nr}}^2\ma{I}_{{M_{\rm r}}} \}$ represents the zero-mean additive white complex Gaussian (ZMAWCG) noise at the relay. The transmitted data symbol from the source is denoted as $s \in \compl$, $\mathbb{E}\{ss^{*}\}=1$. $P_{\rm{s}}$ and $P_{\rm{s,max}}$ are the source transmit power and its maximum allowed values, respectively. ${\ma{u}_{{\rm in}}} \in \compl^{M_{\rm r}} $ represents the {\emph{undistorted}} received signal at the relay. The receiver distortion is denoted as \mbox{$\ma{e}_{{\rm in}} \in \compl^{M_{\rm r}}$} which represents the combined effects of receiver chain impairments, e.g., limited ADC accuracy,  in facing with the high-power self-interference signal. For detailed elaboration on this distortion model please refer to \cite{Day2012, DMBSR:12} and system measurements in \cite{MITTX:08,MITRX:05}. While the aforementioned error is assumed to be ignorable in many classic HD schemes, it plays an important role in our system due to the high power nature of the self-interference. The known, i.e., distortion-free, part of the self-interference signal is then suppressed and the resulting signal is amplified to constitute the relay's output: \footnotemark[1]
\begin{align}
 \ma{r}_{{\rm out}} &=  \ma{u}_{\rm out}   +  \ma{e}_{{\rm out}}, \;\; \ma{u}_{{\rm out}} := \ma{W} \ma{r}_{{\rm supp}}   \label{eq_model_r_out}\\
 \ma{r}_{{\rm supp}} &= \ma{ r}_{{\rm in}} - {\ma{H}}_{{\rm rr}} \ma{u}_{{\rm out}}, \label{eq_model_r_supp}
\end{align}
where $\ma{r}_{{\rm supp}} \in \compl^{M_{\rm r}}$ and $\ma{W} \in \compl^{{M_{\rm r}} \times {M_{\rm r}} }$ respectively represent the interference-suppressed version of the received signal and the relay amplification matrix. The \emph{intended} transmit signal is denoted as $\ma{u}_{{\rm out}}$. Similar to the defined distortion in the receiver chains, we define the transmitter distortion as \mbox{$\ma{e}_{{\rm out}} \in \compl^{M_{\rm r}}$} which represents the effect of limited transmitter dynamic range, \cite{Day2012, DMBSR:12}. As it has been shown, the variance of the distortion components is proportional to the collected power on the receiver antennas (undistorted received signal), for $\ma{e}_{{\rm in}}$, and to the power of the transmit signal prior to DAC module (intended Tx signal), for $\ma{e}_{{\rm out}}$:
\begin{align}
\ma{e}_{{\rm in}}  \sim \mathcal{CN} \left\{ \ma{0}, \beta \text{diag}\Big(\mathbb{E}\left\{\ma{u}_{\text{in}}\ma{u}_{\text{in}}^{{H}}\right \} \Big) \right\}, \label{eq_model_e_in}
\end{align}
and
\begin{align}
\ma{e}_{{\rm out}}  \sim \mathcal{CN} \left \{ \ma{0}, \gamma \text{diag}\Big(\mathbb{E}\left\{\ma{u}_{\rm{out}}\ma{u}_{\rm{out}}^{{H}}  \right \}  \Big) \right\}, \label{eq_model_e_out}
\end{align}
where $\beta ,\gamma \in \real^{+}$ are coefficients respectively relating the undistorted receive and transmit signal covariance to the covariance of the resulting distortion. Please note that the above statistics of the distortion signals differ from the known ZMAWCG signal components, as the variance of the resulting transmit (receive) distortion at each antenna is proportional to the variance of the corresponding transmit (receive) signal. 
  
\subsection {Relay-to-destination communication}
The transmitted signal from the selected relay node passes through the relay to destination channel and constitutes the received signal at the destination:
\begin{align}
 \ma{y} &=  \ma{H}_{{\rm rd}} \ma{r}_{{\rm out}} + \ma{n}_{\rm{d}}, \;\; \hat{s}= \ma{z}^{{H}}\ma{y}, \label{eq_model_y}
\end{align}
where $\ma{y}$ is the received signal at the destination, and $\ma{n}_{\rm{d}}\sim \mathcal{CN} \{ \ma{0}, \sigma_{\rm{nd}}^2{\ma I}_{M_{\rm{d}}}  \}$ is the ZMCSCG noise. The linear receiver filter and the estimated received symbol is denoted as \mbox{$\ma{z}\in\compl^{M_{\rm{d}}}$} and $\hat{s}$, respectively. 

   The transmit power of the relay node is limited by 
\begin{align}
&  \mathbb{E} \{ \|\ma{r}_{{\rm out}}\|_2^2  \}  \leq P_{\rm{r,max}}, \label{eq_model_P_max}
\end{align}
where $P_{\rm{r,max}}$ represents the maximum relay transmit power.  
\mbox{Table I} provides the description of the signal notations to better communicate the defined model. 

\subsection{Distortion loop} \label{discussion:distortionLoop}
In this part we provide an intuitive description of the aforementioned distortion loop, following the defined system model, which makes the subsequent arguments in the paper more clear. As the transmit power from the relay increases, the power of the error components increase in all receiver chains, see (\ref{eq_model_r_in}) in connection to (\ref{eq_model_e_in})-(\ref{eq_model_e_out}). On the other hand, these errors are amplified in the relay process and further increase the relay transmit power, see (\ref{eq_model_r_in}) in connection to (\ref{eq_model_r_supp}) and (\ref{eq_model_r_out}). The aforementioned effect causes a loop which signifies the problem of residual self-interference for the relays with AF process. In the following section, we analyze the aforementioned effect for the defined AF-FD relaying setup with multiple antennas.
